Knowing Who Knows What: Designing Socially Assistive Robots with Transactive Memory System

Transactive Memory System (TMS) is a group theory that describes how communication can enable the combination of individual minds into a group. While this theory has been extensively studied in human-human groups, it has not yet been formally applied to socially assistive robot design. We demonstrate how the three-phase TMS group communication process-which involves encoding, storage, and retrieval-can be leveraged to improve decision making in socially assistive robots with multiple stakeholders. By clearly defining how the robot is gaining information, storing and updating its memory, and retrieving information from its memory, we believe that socially assistive robots can make better decisions and provide more transparency behind their actions in the group context. Bringing communication theory to robot design can provide a clear framework to help robots integrate better into human-human group dynamics and thus improve their acceptance and use.

==> 2_related_work.tex <==
\section{Related Work}
\subsection{Transactive Memory System}
Transactive Memory System (TMS) was first introduced in studying the cognitive interdependence among intimate dyads that two individuals depend on each other's thoughts and generate knowledge (Wegner et. al 1985). TMS was further studied as a group mind theory more broadly beyond dyad couples and used to predict the group behaviors through the communication process among the group members (Wegner 1987). Defined as "a combination of individual minds and the communication among them," TMS consists of two components, i.e., each group member's independent memory system and the communication events among group members that enable the interplay of knowledge (Wegner et. al 1985). The first component, also known as “Who knows what” (Lewis et al., 2007), suggests that transactive memory consists of the knowledge of everyone in the group as well as the location of the knowledge among the group members. The second component of TMS refers to the communication process in forming the transactive memory that consists of three phases, i.e., encoding, storage and retrieval. 

TMS has two types of structures, i.e., differentiation and integration (Wegner et. al 1985). The differentiated structure introduced the distinctions of personal memories in the group. TMS categorized information into higher-order, lower-order information, and location information. Higher order information is the topic, theme, category or sets of lower order information. For example, “fruit” is the higher order information while “apple” is lower order information. Location information is where to find the higher order or lower order information. The theory suggested that members share common higher-order information and location information but possess different lower-order information. The individual can access the lower-order information of their partners through communication, therefore, the group members can be the external memory storage for each other. The integration structure is the process for group members to reach a shared understanding of the topic with initially disparate opinions. Integration could create new perspectives towards the topic which the group members didn’t possess individually. 

TMS is also a social process with assigning the responsibility among the group members. The formation of TMS requires learning of each other's expertise and taking up the responsibility for information. People accept the responsibility for information if they are an expert or if they know that their partner doesn't have the expertise. Therefore, the formation of transactive memory is an automatic social process to delegate responsibility of keeping information to our partners or ourselves, which is affected by what we know about other people's knowledge and what we can expect from them. 


The process of transactive memory is studied in analog of individual memory with respect to three phases of knowledge processing: transactive encoding, transactive storage and transactive retrieval. The three stages provided a framework to study how communication takes place and affect the knowledge processing and generation in each stage. For example, the "generation effect" is commonly observed in the transactive memory encoding stage, that people tend to remember better if they actively generate information rather than passively experience and process it. The communication in group could enable active information generation through discussions and trigger “generation effect,” i.e., people remember better through the active group participation. In addition, effortful communication in the encoding process was found to enhance memory of the group such as analysis, argument, and decision-making. 

In the storage stage, transactive memory can be highly modifiable with the subsequent events and information simplification in the communication process. As shown in the study of social transmission of information, the nature of a story can be modified after sending it to a chain of people. 

In the retrieval stage, interactive cuing could be a factor that leads to the retrieval success, that one person uses a cue from others to recall the full information. Furthermore, based on the finding that contextual information helps with individual memory retrieval, the presence of other group members might provide the context of information encoding and lead to a better retrieval outcome. 


\subsection{TMS and Communciation Factor}
Prior work has studied the communication in TMS from a network perspective and discuss the effects of communication factors on TMS with respect to the group’s timespan (Yan et al., 2021). This work reviewed 64 empirical studies on TMS and the finding revealed the importance of group communication in TMS whose influence is differentiated at the beginning and later stage of the group’s lifespan, i.e., the TMS development in newly formed groups and the TMS utilization in established groups. In the TMS development stage, communication content (expertise information), channels (face-to-face, CMC), qualities (helpfulness, openness, length, closeness) were found to affect the outcome of transactive memory formation in the early stage. In the TMS utilization stage, the finding revealed that information exchange could increase overtime while the effectiveness of information exchange is not guaranteed. In addition, group member relationships and group climates are associated with information sharing in TMS in the established stage, that more information sharing could lead to positive group climate, while negative group climate can reduce the information sharing. The finding from the literature review pointed to the multidimensional network perspective in studying TMS in groups, which situates groups in context and incorporate factors such as technologies, member characteristics, communication styles in studying TMS.

Similarly, Yuan et al., has taken a multilevel network perspective in studying TMS with a focus on social accessibility to expertise providers (Yuan et al., 2010) and interpersonal affective relationship (Yuan et al., 2014). Yuan et al., 2010 investigated the effect of perceived social accessibility, media multiplexity, and expertise awareness on both dyadic and individual levels on the dyadic expertise retrieval outcome (Yuan et al., 2010). The finding suggested that expertise retrieval is more likely to happen when the member knows the other’s expertise better, the expert person is perceived as being more accessible, and more communication channels are available. 

Built on the finding of the previous study, Yuan et al. further studied the effect of awareness, affective ties, and expertise seeking among the group members on expertise retrieval (Yuan et al., 2014). The study conducted a web-based survey among teams within an international organization and found that positive relationship among group members have a positive effect on expertise seeking. The effect is amplified by the awareness of expertise distribution that “having a positive affective tie will increase the positive effect of awareness on expertise seeking from each relationship.” The paper emphasized the individual level construct, i.e., affective ties among the group members and awareness of expertise distribution, in studying TMS in comparison with the group level factors. The paper also suggested that the social network perspective could be explanatory for knowledge management in groups and TMS.

In addition, interpersonal factors were researched by Neff et al. who studied the positive affect on the individual level and group level and their effects on information seeking and sharing among the group members. The result revealed that a positive correlation between the positive affect among the group members and the volume of transactive communications (both information sharing and seeking), as well as a significant relationship between affective homogeneity and information sharing only. The interpersonal constructs were only found to impact the transactive communication outcome, but not the transactive communication processes. 


\subsection{TMS and Individual Memory}
While communication and interpersonal factors can affect the transactive memory of the group, the forming of transactive memory can in turn affects the individual’s memory, through which people make sense of their experience and environment at present (Barnier et al., 2008) as well as create prospective memories for the future (Schacter et al., 2007). This section reviewed literature that studied how the individual memory is shaped through group communication and social interactions.  

Prior research has suggested that human memories are embodied, distributed, or extended in the environment as opposed to being an isolated cognitive process in the brain (Barnier et al., 2008). The paper presented a distributed cognitive framework to study the social memory phenomenon with four factors related to memory sharing: costs and benefits (e.g., memory recalled and forgotten, accuracy of recall, and memory quality), parameters of group influence (e.g., size and type of the group, manner of collaboration, similarity of memories and retrieval strategies, social and motivational factors), the fate of memories (i.e., why some memories died off more quickly than others) and the function of group memory (e.g., defining identity, teaching and communicating, relationship development and maintenance, self and group representation). The distributed cognitive framework is rooted in the social aspect of memory and views external factors as an integrated part of the memory formation and history rather than merely triggers for the internal processes. In this sense, the group memories and the social interactions in the group are essential for individuals to create memories and make sense of self and others along the way of recording our past.   
Under the same vein, the social aspect of memory was studied in terms of collaborative remembering (Hirst et al., 2012). The paper discussed two major ways that conversational remembering would affect the subsequent memory after the conversation: Social Contagion and Retrieval/Reexposure Effect. 

Social contagion is defined as “the spread of information, ideas, or practices via the social network,” and can impose new memories or alter the existing memories of the listener. Social contagion can be modified by cognitive moderators or social-interpersonal moderators. Cognitive moderators discussed in the paper include the consistency between the “contagious” items and the expectation, the length of the information, preference for peripheral/central details, and whether the information is old or new. Furthermore, social moderators could be the relative power status, closeness of the relationship, anxiety level towards negative evaluation, number of speakers, agreement of the speaker, the communication channel (face-to-face versus writing), and the dominance of the speaker. 

Retrieval/Reexpossure effect suggested that the memories can be modified by “reinforcing some memory or inducing forgetting for others.” Retrieval-induced forgetting (RIF) was found to influence both the listener and speaker and were categorized into two types: “within-individual retrieval-inbound forgetting” (WI-RIF) and “socially shared retrieval-inbound forgetting” (SS-RIF) (Cuc et al., 2007). A shared reality can be created with conversational remembering if the speaker is motivated to achieve it with the likelihood that information bias would occur. Overall, the review paper on collaborative memory suggested that remembering is embedded in a social context and the social conversations can shape memories both on the individual level and collective level. 

\subsection{TMS and Collective Recalling}
Besides the theoretical background, prior work has empirically evaluated the communication factors and collective memory outcome (Harris et al., 2011). Harris et al. studied the collaborative remembering among older couples and revealed the communication processes that could facilitate or inhibit the recalling outcome. The studied asked participants to engage in three types of collective recalling tasks: word list recall, personal list recall, and autobiographical interview. The finding revealed a list of factors in the collaborative communication processes such as cueing, response to a cue, mentions of expertise, strategy disagreement, repetitions, acknowledgements, corrections, and elaborations. Among those factors, successful cuing and repetition could contribute to the group remembering, whereas incompatible expertise, corrections and conflicting recalling strategies could diminish the recalling outcome. The result also showed older adult couples have used a mixture of implicit strategies and explicit strategies in the collective recalling tasks. Both types of strategies seem to contribute to the collaborative recalling tasks regardless of if they are explicit or implicit.  

Another study suggested that the shared memories are associated with the personhood of people living with dementia through a co-creative and collective recalling process (Wallace et al., 2013). In this study, one older dyad engaged in a series of jewelry design activities with bespoke probes provided by the research team. The design activities were a way to trigger reminiscence among the couple. The past emotions and memories were manifested in the collective recalling process and materialized in the design artefacts that the couple collectively created. The co-design process evoked the shared memories between the couple and became a sense making process for the individual living with dementia. This study showed that the how one might rebuild their identity and personhood from the collective memory even if their own memory became inaccurate or even got lost. 


==> 3_methods.tex <==
\section{Design Framework}
\subsection{Transactive Memory Process with Robots}
\subsubsection{Memory Encoding Phase}
\subsubsection{Memory Storage Phase}
\subsubsection{Memory Retrieval Phase}

\subsection{Case Study: Transactive Memory with Socially Assistive Robots}

The previous sections summarized the theory of TMS and reviewed literatures studying the effect of communication factors on TMS, the interplay between individual memories and TMS through social interactions, and the process and outcome of collective recalling. While most of the previous TMS research is centered around interpersonal communications, the findings from interpersonal studies on TMS could inform the research on human-machine interactions in memory-related activities, e.g., how the TMS might be formed in the human-machine group, and how the technical artefacts can be designed to support people with memory assistance needs. This case study aims to focus on socially assistive robots and people with traumatic brain injury. 

Socially assistive robots are built with human-like communication styles using natural languages and nonverbal cues, physically embed in the environment and have a certain level of autonomy (Feil-Seifer et al., 2006; Dautenhahn, 2007). In comparison to passively used computers, users’ interaction with socially assistive robots is cooperative and requires the understanding of each other's knowledge (Scassellati, 2002; Görür et al, 2017). Socially assistive robots have been investigated to help with people with traumatic brain injury (TBI) (Matarić, 2009; Matarić, 2017), who often experience short term memory loss and have difficulty remembering new events. Socially assistive robots can serve daily assistant for TBI users, help them keep track of daily activities, that the user can record the events and ask the robot to help them recall the information. 

TMS provides the theoretical background that individual’s memories can be extended in groups with transactive memories. Analog to TMS in humans, TBI users could form transactive memories with socially assistive robots which could assist them with overcoming everyday challenges caused by memory loss. However, it’s unknown how the robot behavior should be designed to better enhance the TMS between the human and machine as well as support the information recalling. Communication is a key component in the process of transactive memory including encoding, storage and retrieval. 


Taking the perspective of socially embedded memory in prior work, social communication was found to be prominent to shape the memory on both the individual and group level (Barnier et al., 2008; Hirst et al., 2012) and affective relationship is positively associated with the TMS retrieval (Yuan et al., 2014). Under the same vein, social interactions could also be critical to form transactive memory between socially assistive robots and TBI users. For example, a more socially oriented conversation might contribute to the affective relationship between the TBI user and the socially assistive robot, which could enhance the transactive memory encoding and retrieval for the TBI user. 


Furthermore, the communication factors studied in the prior work could inform the design factors of the socially assistive robots, such as communication styles, cuing, amount of information exchanges, power status, accessibility of the information provider, communicative strategies, affective ties, etc. (Yuan et al., 2010; Yuan et al., 2014; Yan et al., 2021; Harris et al., 2011). For example, the socially assistive robot in the encoding process could be more conversational to help TBI users narrate events that they would like to share and build up trust and affective ties. In the retrieval stage, the socially assistive robots might need to balance the goal of improving effectiveness of information recalling and the experience of makings sense of the past through the memory recalling.  

